Piecewise-Linear Manifolds for Deep Metric Learning

Unsupervised deep metric learning (UDML) focuses on learning a semantic representation space using only unlabeled data. This challenging problem requires accurately estimating the similarity between data points, which is used to supervise a deep network. For this purpose, we propose to model the high-dimensional data manifold using a piecewise-linear approximation, with each low-dimensional linear piece approximating the data manifold in a small neighborhood of a point. These neighborhoods are used to estimate similarity between data points. We empirically show that this similarity estimate correlates better with the ground truth than the similarity estimates of current state-of-the-art techniques. We also show that proxies, commonly used in supervised metric learning, can be used to model the piecewise-linear manifold in an unsupervised setting, helping improve performance. Our method outperforms existing unsupervised metric learning approaches on standard zero-shot image retrieval benchmarks.

==> tables/algo_box.tex <==
\begin{algorithm}
\KwResult{Projector function $f_{\theta}$}
\KwData{ Train Dataset
$\mathcal{D}:=\left\{\textbf{X}_{L}, Y_{L}\right\}$ with $N$ classes, }
\textbf{Set:} Num. epochs $E$, reassign interval $\mathcal{R}$ , Number of proxies per class $M$

\For{$t \in \{1, \hdots, E\}$ }{
    \textbf{\# Proxy Re-assignment} 
    \item[]
    \If{$ \left( t \% \mathcal{R} == 0\right)$}
    {
    \For{$\textbf{x}_{i} \in \mathcal{D}$ }{
    $\textbf{z}_{i} = f_{\theta}(\textbf{x}_{i})$\;
    }
    \For{$j \in \{1, \hdots, N\}$ }{
    Get $\mathcal{Z}_{j} = \{\textbf{z}_{i} \in \mathcal{Z}_{j}:y_{i} == j, \forall i \}$\;
    $\textbf{p}_{j} = \textrm{K-Means}(\textbf{z}_{j}, M)$\;
    ($\textbf{p}_{j}$ = set of all cluster centers returned by K-Means)\;
    }
    }
    \item[]
    \item[]
    $\mathcal{P} = \cup_{\forall j} \textbf{p}_{j}$\;\\ 
    \item[]
    %\item[]
    \textbf{\# Training}
    \item[]
  \For {\textrm{batch} $\mathcal{B} \in \mathcal{D}$}
  {
  \For{$\{\textbf{x}_{i},y_{i}\} \in \mathcal{B}$}{
     Calculate $\mathcal{L}_{i} =\sum_{j=1}^{N }{\sum_{k=1}^{M }{ \mathcal{L}_{i,j,k}}}$ \;
     using Eq. 2 \& 4\;
     Calculate $\mathcal{L}_{i}^{*} = \sum_{n=1}^{\lvert \mathcal{B} \rvert }{\mathcal{L}_{i,n}^{*} }  $ \;
     where $\mathcal{L}_{i,n}^{*}$ is calculated using Eq. 6\;
    }
    
    $\mathcal{L}_{batch}= \sum_{i=1}^{\lvert \mathcal{B} \rvert}{\mathcal{L}_{i} + \mathcal{L}_{i}^{*} } $ \;

    
      $\theta \leftarrow \theta - \eta_{1} \nabla_{\theta} \mathcal{L}_{batch}$ \;

    
      $\mathcal{P} \leftarrow \mathcal{P} - \eta_{2} \nabla_{\mathcal{P}} \mathcal{L}_{batch}$ \;
      
   
   }
   
   }
   \textbf{Return} $f_{\theta}$ 
\caption{Potential Field based DML. Equation numbers refer to the main paper.} 
\label{alg:pdml} 
\end{algorithm}


==> tables/table_SOP_results.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{1em}
    \begin{tabular}{|l || c  c  c  |}
    \hline
    \multicolumn{1}{|l||}{\textbf{Benchmarks $ \rightarrow$}} & \multicolumn{3}{c|}{\textbf{SOP}} \\ \hline \hline
    % \multicolumn{2}{l|}{Recall@$K$}  &
    Methods $\downarrow$  & 
        R@1 & R@10 & R@100  \\ \hline 
   
    MultiSimilarity~\cite{multisimilarity_dml} & 
        78.2 & 90.5 & 96.0  \\ 
    DiVA~\cite{diva_dml} &
       78.1 & 90.6 & - \\
    SoftTriple~\cite{soft_triplet} &
       78.3 & 90.3 & 95.9  \\
    CircleLoss~\cite{circle_dml} &  
        78.3 & 90.5 & 96.1  \\
     HTL \cite{HTL} &
        74.8 & 88.3 & 94.8  \\ 
%     RLL-H \cite{ranked_list} &
 %       76.1 & 89.1 & 95.4  \\ 
    ProxyGML~\cite{proxy_gml} &  
        78.0 & 90.6 & 96.2  \\ 
    Proxy Anchor~\cite{proxy_anchor} &  
        79.1 & 90.8 & 96.2  \\
      DRML-PA~\cite{DRML} &
       71.5 & 85.2 & 93.0  \\
    MS+DAS~\cite{das_eccv22} &  
        78.2 & 90.3 & 96.0  \\
    PA+niV~\cite{vonMF_dml} &  
        79.2 & 90.4 & -  \\ \hline
      
    \textbf{Ours} &
     \textbf{79.8} & \textbf{90.5} & \textbf{96.4}   \\ 
        \hline
    
    \end{tabular}
    \vspace{0.1mm}
    \caption{
        Comparison of the Recall@$K$ ($\%$) on the SOP dataset achieved by our method with state-of-the-art baselines using an Inception with batch normalization~\cite{Batchnorm} backbone and a 512 dimensional embedding.}
    \label{tab:eval_sop}
    \vspace*{-4mm}
\end{table}

==> tables/table_params.tex <==
\begin{table*}[!h]
    \centering
    \setlength{\tabcolsep}{1em}
    \begin{tabular}{|l| c | c | c | c | c |}
    \hline
    \textbf{Dataset} $\rightarrow$ &\multicolumn{2}{c|}{\textbf{CUB-200-2011}} & \multicolumn{2}{c|}{\textbf{Cars-196}} & \textbf{SOP} \\ \hline
    Arch/Dim & R50/512 & IBN/512 & R50/512 & IBN/512 & IBN/512 \\ 
    \hline 
    $\alpha$ & 10 & 5 & 10 & 5 & 1\\
    $\delta $ &  0.2 & 0.2 & 0.2 & 0.2 & 0.1 \\
       $\mathcal{R}$  &  5 & 5 & 5 & 5 & 5\\
        $M$ & 35 & 35 & 30 & 30 & 30\\
        \hline 
        optimizer & AdamW & AdamW & AdamW & AdamW & AdamW \\
        learning rate & $1e^{-4}$ & $1e^{-4}$ & $1e^{-4}$ & $1e^{-4}$ & $1e^{-4}$\\
        weight decay & $1e^{-4}$ & $5e^{-4}$ & $1e^{-4}$ & $5e^{-4}$ & $5e^{-4}$\\
        BN freeze & Yes & Yes & Yes & Yes & No\\
        Warm-up & 1 & 1 & 1 & 1 & 0\\
        lr-scheduling & None & None & None & None & None \\
        lr for proxies & 0.01 & 0.01 & 0.01 & 0.01 & 0.01\\ \hline
    \end{tabular}
    \caption{Hyperparameter details for Potential Field based DML for experiments described in Section 4 of the main paper.}
    \label{tab:hyper_param1}
\end{table*}
